Tractable Graph Structures in EFX Orientation

Since its introduction, envy-freeness up to any good (EFX) has become a fundamental solution concept in fair division of indivisible goods. Its existence remains elusive -- even for four agents with additive utility functions, it is unknown whether an EFX allocation always exists. Unsurprisingly, restricted settings to delineate tractable and intractable cases have been explored. Christadolou, Fiat et al.[EC'23] introduced the notion of EFX-orientation, where the agents form the vertices of a graph and the items correspond to edges, and an agent values only the items that are incident to it. The goal is to allocate items to one of the adjacent agents while satisfying the EFX condition. Building on the work of Zeng and Mehta'24, which established a sharp complexity threshold based on the structure of the underlying graph -- polynomial-time solvability for bipartite graphs and NP-hardness for graphs with chromatic number at least three -- we further explore the algorithmic landscape of EFX-orientation using parameterized graph algorithms. Specifically, we show that bipartiteness is a surprisingly stringent condition for tractability: EFX orientation is NP-complete even when the valuations are symmetric, binary and the graph is at most two edge-removals away from being bipartite. Moreover, introducing a single non-binary value makes the problem NP-hard even when the graph is only one edge removal away from being bipartite. We further perform a parameterized analysis to examine structures of the underlying graph that enable tractability. In particular, we show that the problem is solvable in linear time on graphs whose treewidth is bounded by a constant and that the complexity of an instance is closely tied to the sizes of acyclic connected components on its one-valued edges.

==> RW-additional.tex <==
\subsection*{Additional related work}The subject of fair division is vast. We point the reader to the surveys \cite{mishra2023fair/survey} and \cite{amanatidis2023fair/survey}. In addition to the papers referred earlier, we can point to a few others that have made significant contributions to the study of EFX. 

Plaut et al.~\shortcite{PR20} shows that EFX allocations exist if all agents have the same valuation function. Mahara~\shortcite{Mahara23/journal} extended this result to two {\it types of agents}, that is, every agent has one of two valuation functions which can be arbitrary. Gorantla et al.~\shortcite{GorantlaMarwaha23} consider different additive valuations, but for at most two types of items.  Amanatidis et al.~\shortcite{AmanatidisBFHV21/journal/tcs} consider bi-valued valuation functions. Another work of a similar nature is that of Babaioff et al.\shortcite{Babaioff2020FairAT} which considers submodular {\it dichotomous} valuations, in which the marginal value of any item relative to a set is either $0$ or $1$. Hosseini et al.~\shortcite{HosseiniSVX21} consider {\it lexicographic} preferences, where the value of a single item is greater than the total value of all items that are less preferred. 


\paragraph{Beyond \EFX orientation.} The graphical setting has been extended to study EF1 and EF~\cite{MisraSethia/ADT24} as well. Deligkas et al.~\shortcite{Deligkas/EFX-EF1-orientations} studies primarily the question of EF1 orientation for hypergraphs and explores the parameterized complexity of EFX orientation. They also strengthen the hardness result of \cite{christodoulou_fair_2023} by showing that the \EFX orientation problem NP-complete even on graphs with constant-sized vertex cover and additive symmetric valuations. Furthermore, for multi-graphs, the NP-hardness extends to instances with only a constant number of agents, 8. Chandramouleeswaran et al.~\shortcite{Chandramouleeswaran/FairDivisionVariableSetting} also study EF1 allocation in the multi-graph setting in relation to problem of EF1 restoration.

\paragraph{Charity}
Caragiannis et al. \shortcite{Caragiannis19/EFX-Charity} initiated the research of finding desirable EFX allocations
that satisfy certain properties, such as maximizing the Nash social welfare, where some goods remain unallocated, i.e the {\it charity} bundle. There has been several follow-up work that have reduced the number of items in the charity bundle, ~\cite{Chaudhury21a},\cite{Chaudhury21b} \cite{Akrami22a},\cite{Berendsohn/MFCS17}, culminating in Berger et al.~\shortcite{BergerCohenFeldmanFiat22} showing that for four agents, 
 giving at most one good to charity is enough.


\paragraph{Chores}Work on EFX allocation for chores has caught steam. Recently, \cite{Christoforidis24/EFX-chores} showed that an EFX allocation for chores need not exist under general cost functions. They present a construction
with three agents in which no bounded approximation exists. Moreover, deciding 
if an EFX allocation exists for an instance with three agents and superadditive costs is NP-complete. 


\paragraph{Intractibility} Goldberg et al.\shortcite{Goldberg/EFX-PLS} study the intractability of EFX with just two agents, and find that computing an EFX allocation for two identical agents with submodular valuations is PLS-hard. Essentially they show that the problem becomes intractable as the valuations become more general. 

\paragraph{Graphical fair division} This is a fast growing topic in which several different fairness criterion, be it comparison based or share-based have been studied: conflict-free fair division~\cite{Chiarelli2022fair}~\cite{Gupta/journal/Budget-cinflict-free}, connected fair division~\cite{deligkas2021parameterized}, compact fair division~\cite{madathil2023fair}, gerrymandering on planar graphs~\cite{dippel2023gerrymandering} are just a few. Graph based EFX allocations is an addition to this body of work. 


==> background.tex <==
\subsection*{Our setting and related work.} In this article, we investigate the problem of allocating $m$ indivisible goods among $n$ agents in the graphical setting as introduced by Christodoulou et al.~\shortcite{christodoulou_fair_2023}. The agents are represented as vertices of a graph and the items are represented by the edges. The agents view the items (i.e edges) they are not incident to as {\it irrelevant}, and thus value them as 0. We study the EFX allocation question for a class of valuation functions associated with a graph. Christodoulou et al.~\shortcite{christodoulou_fair_2023} considered both possibilities: an allocation that allows irrelevant items to be allocated as well as that which does not (calling it an \EFX~{\it orientation}). They showed that while an \EFX allocation always exists and can be computed in polynomial time for general valuation functions, computing an \EFX orientation is NP-complete even when valuations are symmetric, that is agents that share an edge value it equally.

Since \cite{christodoulou_fair_2023} this setting has been subsequently explored by several works that have extended the \EFX allocation question to related settings. Specifically, Amanatidis et al.~\shortcite{ApproxEFX-A/EC24} study approximate graphical EFX allocations showing that a 2/3-\EFX allocation\hide{\footnote{An allocation is said to $\alpha$-\EFX if for a given $\alpha \in (0,1)$, the following holds: for each pair of agents $i,j$, and each item $x\in A_i$, agent $v_j(A_j) \geq \alpha\cdot v_j(A_i \setminus\!x)$. \todo{should we define this? we don't use it at all ourselves...}}} always exists and can be efficiently computed for agents with additive valuation functions in Christodoulou's multi-graph setting. Zhou et al.~\shortcite{10.24963/ijcai.2024/338} show that \EFXp orientation always exists and can be found in polynomial-time, drawing a contrast with \EFX orientation which may not always exist,~\cite{christodoulou_fair_2023}. Moreover, they initiate work on graphical EFX on {\it chores}, also studied by \cite{HsuKing24/EFX-O-chores}; and {\it mixed manna}, which is a generalization of both.
Most related to our work are that of Zeng et al.~\shortcite{MehtaZeng2024structureefxorientationsgraphs}, Afshinmehr et al.~\shortcite{Afshinmehr/EFX-A-O-bipartite}, and Bhaskar et al.~\shortcite{Bhaskar24/EFX-A-multigraph}. Zeng et al.~\shortcite{MehtaZeng2024structureefxorientationsgraphs} study the problem of {\it strong \EFX orientation}, where the goal is to decide if a given graph will have an \EFX orientation irrespective of the valuation function. They establish a non-obvious connection with the chromatic number of the graph, and in the process define a complete characterization of strong EFX orientation when restricted to binary valuations. Specifically, they demonstrate the centrality of bipartiteness in the tractability of the EFX problem. Other papers, such as \cite{Bhaskar24/EFX-A-multigraph}, \cite{Afshinmehr/EFX-A-O-bipartite} have since focused on bipartite graphs or multi-graphs to find positive results.
Afshinmehr et al.~\shortcite{Afshinmehr/EFX-A-O-bipartite} study \EFX allocation and orientation questions when restricted to bipartite multi-graphs with additive valuations and show that the former is always guaranteed to exist but the latter may not even for simple instances of multi-trees. They show that that orientation question is NP-hard even when the number of agents is a constant and study parameters such as the maximum number of edges between two vertices and the diameter of the graph. 
Bhaskar et al.~\shortcite{Bhaskar24/EFX-A-multigraph} study EFX allocation in bipartite multi-graphs, multi-tree, and multi-graphs with bounded girth for {\it cancellable monotone valuations}.\footnote{A monotone valuation function is cancellable if for a subset of items $S, T $ and item $x \in S \cup T$, if $v(S) \geq v(T)$, then $v(S \cup \{x\}) \geq v(T \cup \{g\})$.} 

Note that the aforementioned graphical setting should not be confused with the one studied by Payan et al. \shortcite{PayanSV23} where like us, the vertices are agents, however the graph is used to relax fairness notions such that a fairness condition (such as EF, EF1, EFX) only need to be satisfied between pairs of vertices that share an edge. 


==> hardness.tex <==
\subsection{Hardness for binary symmetric valuation}

In this section, we describe a \Ma{pair of reductions, \Cref{thm:edgeoct2} and ??,}\ma{Only 1 hardness result in this section} which proves that the tractability noted in the previous section is in essence optimal.

\begin{theorem} \label{thm:edgeoct2}
    \EFXO is W[1]-hard with respect to the number of 1-components with more than five vertices even on inputs that have \EOCT equal to 2 \hide{and have a binary valuation}. This also holds on inputs with \EOCT equal to 1 when all edges except one have binary values.
\end{theorem}
    \il{If we phrase it this way, then shouldn't that proof come first ?}
    \Ma{We use a similar reduction to the proof of \Cref{thm:wone_complex_components}, reducing from multicolored independent set.}
    Suppose that we are given an instance of MIS, consisting of a graph $G'$, an integer $k$, and a $k$-partition $V_1,\dots,V_k$ of $V(G')$.
    We describe the graph $G$, result of the reduction, starting with its 1-graph.
    For each color $i$ in our MIS instance we produce a path $P_i$ on $4 |V_i|$ vertices.
    Each vertex $u \in V_i$ corresponds to four vertices of the path denoted $u_1$ to $u_4$.
    (We aim to represent the choice of $u \in V_i$ in MIS by rooting $P_i$ in $u_2$ or $u_4$.)
    Additionally, for each vertex $u \in V_i$ we produce an auxiliary path $Q_u$ on five vertices $x_{u,1}$ to $x_{u,5}$.
    Aside from the described vertices, the instance also contains four isolated vertices $a_1$, $a_2$, $b_1$, and $b_2$.
    We now add 0-edges.
    For each vertex $u$ we add 0-edges $u_2 a_1$ and $u_2 a_2$.
    We also add 0-edges $x_{u,3} b_1$, $x_{u,3} b_2$, and $u_3 x_{u,2}$.
    For every $v \in N(u)$ we add the 0-edge $x_{u,4} v_3$.
    \begin{figure}[ht]
        \centering
        \includegraphics[scale=1.1,page=1]{figures/oct_hardness.pdf}
        \caption{
            Result representing a connection between $u$ and $v$.
            Dashed top gray area represents $u$ on path for its color together with its auxiliary path $Q_u$ while the dotted bottom gray area shows only part of a path that represents $v$.
            Full and empty vertices show the bi-partition.
        }%
        \label{fig:oct_one_connection}
    \end{figure}

    We will later add a gadget over $\{a_1,a_2,b_1,b_2\}$ to enforce the following property, for now we just assume it.
    \begin{definition}\label{def:good}
        We say an EFX orientation of $G$ is \emph{good} if every vertex with a 0-edge to either both $a_1$ and $a_2$ or both $b_1$ and $b_2$ is assigned at least one of these 0-edges.
    \end{definition}

    \begin{lemma} \label{lem:reductionindependence}
        In a good orientation of $G$, for all edges $uv \in E(G)$, if $u_2$ or $u_4$ are chosen as a root then neither $v_2$ nor $v_4$ can be chosen as a root.
    \end{lemma}
    \begin{proof}
        Assume $u_2$ or $u_4$ get no 1-items, say $u_2$ (argument for $u_4$ is identical).
        Then $u_3$ must get at most one item, otherwise $u_2$ would strongly envy $u_3$.
        Hence $u_3 x_{u,2}$ must be oriented away from $u_3$.
        Since the orientation is good, $x_{u,3}$ is assigned a 0-edge so neither $x_{u,2}$ nor $x_{u,4}$ can be roots of $Q_u$.
        Now $x_{u,2}$ got a 0-edge so if $x_{u,1}$ or $x_{u,3}$ were roots they would be strongly envious of $x_{u,2}$.
        Therefore, $Q_u$ must be rooted at $x_{u,5}$.
        Again, $x_{u,4}$ must get only one item, $x_{u,4} v_3$ is oriented away from $x_{u,4}$, so $v_3$ gets a 0-edge.
        Now if $v_2$ or $v_4$ were chosen as roots of their path they would be envious of $v_3$.
    \end{proof}

    \begin{lemma}
        There exists a good EFX orientation of $G$ if and only if there exists a multicolored independent set of $G'$.
    \end{lemma}
    \begin{proof}
        We first assume we have a solution $S$ to our instance of MIS.
        For each $i \in [k]$ let $\{v\} = S \cap V_i$ we choose $v_2$ as the root for $P_i$ in our solution to \EFXO.
        Additionally, for each $v \in V(G')$ we choose $x_{v,5}$ as a root for $Q_v$ if $v \in S$ and $x_{v,1}$ if $v \notin S$.
        Since $S$ is multicolored we choose exactly one root from each $P_i$.
        Since $S$ is an independent set for any edge $uv$ the solution does not contain both $u$ and $v$.
        If $u \in S$ we rooted in $x_{u,5}$ but not in $v_2$ and if $v \in S$ we rooted in $v_2$ and in $x_{u,1}$ because $u \notin S$.
        In both cases the edge $x_{u,4} v_3$ will not cause envy.

        Conversely, we assume we have a good orientation of $G$, and let the set of roots be $S'$.
        For each color $i$ we find the vertex $u$ that satisfies $u_2 \in S'$ or $u_4 \in S'$ and add it to our solution $S$ to MIS.
        Every EFX orientation has at least one root in each component, and in particular in each $P_i$ so $S$ is colorful.
        Suppose that there exists an edge $uv \in E(G')$ such that $u \in S$ and $v \in S$.
        By construction of $S$ this would mean that $x \in \{u_2,u_4\}$ and $y \in \{v_2,v_4\}$ were chosen as roots.
        But this contradicts \Cref{lem:reductionindependence} for the edge $xy$.
        Therefore, $S$ is an independent set.
    \end{proof}

    It remains to describe a gadget, $H$, on $a_1$, $a_2$, $b_1$, and $b_2$ that ensures that all EFX orientations of $G \cup H$ are good. We will give two possibilities.

    The first possible gadget is simply two 1-edges: $a_1a_2$, and $b_1b_2$.
    Since every edge can be oriented towards only one of its two endpoints, one of $a_1$ or $a_2$ will be assigned the 1-edge $a_1a_2$.
    As $a_1$ and $a_2$ are twins (have identical neighborhoods), suppose without loss of generality that we assigned the 1-edge to $a_1$.
    Then $a_2$ will be envious of $a_1$ if $a_1$ receives any 0-edges.
    Therefore, all 0-edges incident on $a_1$ must be oriented away from $a_1$, and hence, any vertex with a 0-edge to $a_1$ will be assigned a 0-edge.
    The same argument applies to $b_1$ and $b_2$.

    The second possible gadget is slightly more complicated.
    Again we have two 1-edges, this time $a_1b_1$ and $b_2a_2$.
    Additionally we have the edge $b_1b_2$ valued at $m$ where $0 < m < 1$.
    We consider the possible orientations of the edges between $a_1$, $a_2$, $b_1$, and $b_2$.
    By symmetry we can assume that the $m$ valued edge is directed from $b_1$ to $b_2$.
    Furthermore, if $a_2b_2$ was oriented towards $b_2$, then $b_2$ would get two items while $a_2$ would have only 0-items so $a_2$ will be envious of $b_2$, see (\subref{fig:oct_one_gadgets_d}.I) of \Cref{fig:oct_one_gadgets}.
    So $a_2b_2$ must be oriented towards $a_2$.
    We can now consider the two cases for the orientation of $a_1b_1$.
    \begin{description}
        \item[Case 1:] Towards $b_1$, see (\subref{fig:oct_one_gadgets_d}.II) of \Cref{fig:oct_one_gadgets}.
            The vertex $a_1$ may be assigned 0-edges but will have a bundle of value zero so will envy $b_1$ unless $b_1$ gets no 0-items, i.e., all 0-edges incident on $b_1$ are directed away from it.
            Furthermore, $b_2$ gets a bundle with value only $m < 1$, so similarly, $b_2$ will envy $a_2$ unless $a_2$ gets no 0-items.
        \item[Case 2:] Towards $a_1$, see (\subref{fig:oct_one_gadgets_d}.III) of \Cref{fig:oct_one_gadgets}.
            The vertex $b_1$ gets no items so both $a_1$ and $b_2$ must get no 0-items.
    \end{description}
    This completes the proof of \Cref{thm:edgeoct2}. 

\begin{figure}[ht]
    \centering
    \hfill
    \begin{subfigure}{0.18\textwidth}
        \centering
        \includegraphics[page=3,scale=1.1]{oct_hardness.pdf}
        \subcaption{}
        % \subcaption{\EFXO instance is created by 1-to-1 mapping; note that labels on left two vertices are swapped to accommodate planarity.}%
        \label{fig:oct_one_gadgets_a}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\textwidth}
        \centering
        \includegraphics[page=4,scale=1.1]{oct_hardness.pdf}
        \subcaption{}
        \label{fig:oct_one_gadgets_b}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\textwidth}
        \centering
        \includegraphics[page=5,scale=1.1]{oct_hardness.pdf}
        \subcaption{}
        \label{fig:oct_one_gadgets_c}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.41\textwidth}
        \centering
        \includegraphics[page=6,scale=1.1]{oct_hardness.pdf}
        \subcaption{}
        \label{fig:oct_one_gadgets_d}
    \end{subfigure}
    \hfill
    % \includegraphics[scale=1.1,page=3]{oct_hardness.pdf}
    \caption{
        (\subref{fig:oct_one_gadgets_a}) A construction with Edge-OCT 2 that forces a good \EFXO, see \Cref{def:good}.
        (\subref{fig:oct_one_gadgets_b}) ...
        (\subref{fig:oct_one_gadgets_c}) A construction with Edge-OCT 1 that forces a good \EFXO.
        (\subref{fig:oct_one_gadgets_d}) A case analysis for the Edge-OCT 1 construction. Arrows pointing away show forced direction for respective 0-edges.
    }%
    \label{fig:oct_one_gadgets}
\end{figure}


==> intro-basic.tex <==


\section{Introduction}

The fair division of resources is a classical problem with deep roots in economics, game theory, and computer science. While fair division of divisible goods—such as land, time, or money—allows for precise proportional splits, the problem becomes significantly more challenging when dealing with indivisible goods, like houses, tasks, or family heirlooms in an inheritance. These goods cannot be split without losing their value, making it difficult to guarantee fairness.

A key challenge in fair division of indivisible goods is that traditional fairness concepts, like proportionality and envy-freeness, may not be attainable even in the simplest scenarios, such as one more agent than items. To address these challenges, researchers have introduced relaxed fairness criteria such as {\it envy-free up to one good} (EF1) \cite{Budish11}, where the goal is to allocation of $m$ indivisible goods among $n$ agents $A_1, \ldots, A_n$ in a manner that for every pair of agents $i$ and $j$, there exists an item $x \in A_i$ such that agent
$j$ does not value $A_i\sm \{x\}$ higher than $A_j$, its own assignment. 
Such allocations are known to always exist, and can be found by the {\it round-robin} protocol~\cite{Caragiannis-EFX/journal} or {\it envy-cycle elimination} protocol~\cite{Lipton04}. In certain scenarios, an EF1 solution can manifest in an absurd unrealistic manner, as demonstrated by the following example: two siblings fighting over their inheritance are not likely to be satisfied if the older gets the family home and grandfather's watch and the younger sibling gets the car, even though the latter is said to be EF1-happy because the removal of the home would make the younger like their bequest better than of the sibling's. Strengthening the condition Caragiannis et al.~\shortcite{Caragiannis-EFX/journal} introduced {\it envy-freeness up to any good} (EFX), where the goal is to create an allocation $A_1, \ldots, A_n$ where for every pair of agents $i$ and $j$, we have that for {\it any} item $x \in A_i$, agent
$j$ values $A_j$ at least as much as $A_i\sm \{x\}$.\footnote{The precise definition in \cite{Caragiannis-EFX/journal} was that of {\it envy-freeness up to any positively-valued good} ~(\EFXp): For any item 
 $x\in A_i$ that agent $j$ values as strictly positive, we have that $j$ values $A_j$ at least as much as $A_i\sm \{x\}$.} In the short time since its introduction~\cite{Caragiannis-EFX/journal}, there has not been a shortage of work directed at solving the EFX problem. In particular, \cite{PR20} show that EFX allocations exist for two agents for general valuations or when they share the same ordinal ranking of goods. A significant breakthrough was attained by Chaudhury et al.~\shortcite{Chaudhury24} which shows that EFX always exists for three
agents when the valuations are additive, and it was later extended to more
general valuations but at the cost of leaving some items unassigned (i.e {\it charity}) Berger et al. \shortcite{BergerCohenFeldmanFiat22} and Akrami et al.~\shortcite{AkramiAlonChaudhury/EC23}.


Due to \cite{Mahara24/journal} it is also known that EFX allocations exist for arbitrary allocations if the number of goods is at most 3
more than the number of agents, that is $m \leq n+3$. Beyond this, the problem has proven to be highly elusive to pin-down \hide{in terms of its computational complexity} even for four agents and additive valuations.  Procaccia in his oft-cited article ``Fair Division’s Most Enigmatic Question"~\cite{Procaccia/article/ACM} has called this a ``major open question" in fair division. 

In light of this problem's difficulty, many works have explored the problem under various restrictions and one of these is the focus of our work. 

\input{background}
\input{RW-additional}

